Graph Planning with Expected Finite Horizon

Graph planning gives rise to fundamental algorithmic questions such as shortest path, traveling salesman problem, etc. A classical problem in discrete planning is to consider a weighted graph and construct a path that maximizes the sum of weights for a given time horizon $T$. However, in many scenarios, the time horizon is not fixed, but the stopping time is chosen according to some distribution such that the expected stopping time is $T$. If the stopping time distribution is not known, then to ensure robustness, the distribution is chosen by an adversary, to represent the worst-case scenario. A stationary plan for every vertex always chooses the same outgoing edge. For fixed horizon or fixed stopping-time distribution, stationary plans are not sufficient for optimality. Quite surprisingly we show that when an adversary chooses the stopping-time distribution with expected stopping time $T$, then stationary plans are sufficient. While computing optimal stationary plans for fixed horizon is NP-complete, we show that computing optimal stationary plans under adversarial stopping-time distribution can be achieved in polynomial time. Consequently, our polynomial-time algorithm for adversarial stopping time also computes an optimal plan among all possible plans.

==> figures/counterexample.tex <==

\begin{example}\label{ex:memory-fixed-T}
Consider the graph of \figurename~\ref{fig:cycle-memory}
with $\abs{V} = n+1$ vertices, and time bound $T = k \cdot n + 1$ (for some constant $k$).
The optimal plan from $v_0$ is to repeat $k$ times the cycle $v_0,v_1,\dots,v_{n-1}$
and then switch to $v_n$. This path has value $1$, and all other path have lower
value: if only the cycle $v_0,v_1,\dots,v_{n-1}$ is used, then the value is at most $0$,
and the same holds if the cycle on $v_n$ is ever used.
The optimal plan can be represented by a Mealy machine of size $O(T / \abs{V})$
that counts the number of cycle repetitions before swithing to $v_n$.
A Moore machine requires size $T$ as it needs a new memory state at evcery step
of the plan
\end{example}



\begin{figure}[!tb]
  \begin{center}
    \hrule
      \input{figures/cycle-memory.tex}
    \hrule
      \caption{A weighted graph (with $n+1$ vertices) where the optimal path (of length $T = k \cdot n + 1$)
is not simple: at $v_0$, the optimal plan chooses $k$ times the edge $(v_0,v_1)$, and then the edge $(v_0,v_n)$. \label{fig:cycle-memory}}
  \end{center}
\end{figure}


\begin{figure}[!tb]
  \begin{center}
    \hrule
      \input{figures/mult-cycle-memory.tex}
    \hrule
      \caption{Three loops of respective length $L_1 = 6 = 2\cdot 3$, $L_2 = 10 = 2\cdot 5$, and $L_3 = 15 = 3 \cdot 5$.
For $T= 32 = 6 + 10 +15 +1$, the optimal plan needs to visit each cycle once. \label{fig:mult-cycle-memory}}
  \end{center}
\end{figure}


\begin{example}\label{ex:memory-fixed-T-multiple-cycles}
In the example of \figurename~\ref{fig:mult-cycle-memory} the optimal plan needs 
to visit several different cycles, not just repeating a single cycle and possible 
swithcing only at the end. The graph consists of three loops on $v_0$ 
with weights~$0$ and respective length $6$, $10$, and $15$, and an edge to $v_1$
with weight $1$. For $T = 6 + 10 + 15 + 1$, the optimal plan has value $1$ and
needs to stop exactly when reaching $v_1$ (to avoid the negative self-loop on $v_2$).
It is easy to show that the remaining length $T-1 = 31$ can only be obtained by visiting
each cycle once: as $31$ is not an even number, the path has to visit a cycle
of odd length, thus the cycle of length $15$; analogously, as $31$ is not a
multiple of $3$, the path has to visit the cycle of length $10$, etc.
This example can be easily generalized to an arbitrary number of cycles by using
more prime numbers.
\end{example}





